Geometric IR subtraction for real radiation

A scheme is proposed for the subtraction of soft and collinear divergences present in massless real emission phase space integrals. The scheme is based on a local slicing procedure which utilises the soft and collinear factorisation properties of amplitudes to produce universal counter-terms whose analytic integration is relatively simple. We propose that this scheme can be promoted to a fully local subtraction method. As a first application the scheme is applied to establish a general pole formula for final state real radiation at NLO and NNLO in Yang Mills theory for arbitrary multiplicities. All required counter-terms are evaluated to all orders in the dimensional regulator in terms of $\Gamma$ - and ${}_pF_q$ hypergeometric - functions. As a proof of principle the poles in the dimensional regulator of the $H\to gggg$ double real emission contribution to the $H\to gg$ decay rate are reproduced.

==> Limits.tex <==
\subsection{Asymptotic Phase Space Measures}
%In the following section we will provide explicit expressions for the differential phase space volumes associated to all NNLO singular limits given in eq.(\ref{eq:limits}). 
%To keep the analytic integration of counterterms as simple as possible we will take subsequent limits in the parameters $a_{i},a_{ij},b_{ij}$ and $b_{ijk}$. In this way we can guarantee that the counterterms depend only logarithmically on the cut-off parameters. 
%
In the following we will fix, for ease of readibility but without loss of generality, the indices $i,j,k,..$ to be integer valued. Further we have set $Q^2=1$ (which here is equivalent to promoting the parameters $b_{ij..}$ to a squared energy scale, while keeping the parameters $a_{i..}$ dimensionaless). 

All further singularities will be overlaps of these limits and those already present at NLO. The triple collinear-double-soft measure is given for instance by:
We then end up with the following list of different asymtptotic phase space elements:
% \bea
%   \{S_1^{(2,3)}\}&:\qquad  &\d\Phi_{S_{1}}^{(2,3)}(a_{1},s_{23})\nn\\
%   \{C_{12}\}&:\qquad  &\d\Phi_{C_{12}}(b_{12}Q^2)\nn\\
%   \{S_{34}\}&:\qquad  &\d\Phi_{S_{34}}^{(1,2)}(a_{34},s_{12})\nn\\
%   \{C_{134}\}&:\qquad  &\d\Phi_{C_{134}}(b_{134}Q^2)\nn\\
%   \{C_{12},S_1^{(2,3)}\} &:\qquad  &\d\Phi_{C_{12}S_1}(b_{12}Q^2,a_1)\nn\\
%   \{C_{13}, S_4^{(2,3)}\} &:\qquad  &\d\Phi_{C_{13}}(b_{13}Q^2)\,\d\Phi_{S_{4}}^{(2,z_3\t{13})}(a_{1},z_3s_{\t{13}2})\nn\\  
%   \{C_{13}, C_{24}\}&:\qquad  &\d\Phi_{C_{13}}(b_{13}Q^2)\,\d\Phi_{C_{24}}(b_{24}Q^2)\nn\\
%   \{C_{134},C_{13}\}&:\qquad  &\d\Phi_{C_{\t{13}4}}(b_{134}Q^2)\,\d\Phi_{C_{13}}(b_{13}Q^2)\nn\\
%   \{C_{13},S_{34}^{(1,2)}\} &:\qquad  & \d\Phi_{C_{13}S_{3}}(b_{13}Q^2,a_{34})\,\d\Phi_{S_4}^{(2,\t{13})}(a_{34}-z_3,s_{\t{13}2})\nn\\
%   \{C_{134},S_3^{(1,4)}\}&:\qquad  &\d\Phi_{C_{14}}(b_{134}Q^2)\,\d\Phi_{S_3}^{(1,4)}(a_3,s_{13})\nn\\
%   \{C_{134},S_4^{(2,3)}\}&:\qquad  &\d\Phi_{C_{13}}(b_{134}Q^2)\,\d\Phi_{C_{\t{13}4}S_4}(b_{134}Q^2-s_{13},z_3 a_4)\nn\\  
%   \{C_{34},S_{34}^{(1,2)}\}&:\qquad  & \d\Phi_{C_{34}}(b_{34}Q^2)\,\d\Phi_{S_{\t{34}}}^{(1,2)}(a_{34},s_{12})\nn\\
%   \{C_{134},S_{34}^{(1,2)}\}&:\qquad  &\d\Phi_{C_{134}S_{34}}(b_{134}Q^2,a_{34})\nn\\
%   \{C_{13}, C_{24},S_3^{(1,4)}\}&:\qquad  & \d\Phi_{C_{13}S_3}(b_{13}Q^2,a_3)\,\d\Phi_{C_{24}}(b_{24}Q^2)\nn\\
%   \{C_{13}, C_{24},S_{34}^{(1,2)}\}&:\qquad  & \d\Phi_{C_{13}S_3}(b_{13}Q^2,a_{34}-z_4)\,\d\Phi_{C_{24}S_4}(b_{24}Q^2,a_{34})\nn\\
%   \{C_{34},S_{34}^{(1,2)},S_{3}^{(1,4)}\}&:\qquad  & \d\Phi_{C_{34}S_3}(b_{34}Q^2,a_3)\,\d\Phi_{S_{\t{34}}}^{(1,2)}(a_{34},s_{12})\nn\\
%   \{C_{134},C_{13},S_{3}^{(1,4)}\}&:\qquad  &\d\Phi_{C_{\t{13}4}}(b_{134}Q^2) \d\Phi_{C_{13}S_3}(b_{13}Q^2,a_3)\nn\\
%   \{C_{134},C_{13},S_{4}^{(2,3)}\}&:\qquad  & \d\Phi_{C_{\t{13}4}S_4}(b_{13}Q^2,z_3a_4)\,\d\Phi_{C_{13}}(b_{134}Q^2)\nn\\
%   \{C_{134},C_{13},S_{34}^{(1,2)}\}&:\qquad  & \d\Phi_{C_{\t{13}4}S_4}(b_{134}Q^2,a_{34})\,\d\Phi_{C_{13}S_3}(b_{13}Q^2,a_{34}-z_4)\nn\\  
%   \{C_{134},C_{34},S_{34}^{(1,2)}\}&:\qquad  & \d\Phi_{C_{1\t{34}}S_{\t{34}}}(b_{134}Q^2,a_{34})\,\d\Phi_{C_{34}}(b_{34}Q^2)\nn\\
%   \{C_{134},S_{34}^{(1,2)},S_3^{(1,4)}\}&:\qquad  & \d\Phi_{C_{14}S_4}(b_{134}Q^2,a_{34})\,\d\Phi_{S_3}^{(1,4)}(a_3,s_{14})\nn\\
%   \{C_{134},S_{34}^{(1,2)},S_4^{(2,3)}\}&:\qquad  & \d\Phi_{C_{13}S_3}(b_{134}Q^2,a_{34})\,\d\Phi_{C_{14}S_4}(b_{134}Q^2-s_{14},a_4z_3)\nn\\
%   \{C_{13},S_{34}^{(1,2)},S_3^{(1,4)}\} &:\qquad  & \d\Phi_{C_{13}S_{3}}(b_{13}Q^2,a_{3})\,\d\Phi_{S_4}^{(2,\t{13})}(a_{34},s_{\t{13}2})\nn\\
%   \{C_{13},S_{34}^{(1,2)},S_4^{(2,3)}\} &:\qquad  & \d\Phi_{C_{13}S_{3}}(b_{13}Q^2,a_{34})\,\d\Phi_{S_4}^{(2,z_3\t{13})}(a_{4},z_3s_{\t{13}2})\nn\\
%   \{C_{13}, C_{24},S_{34}^{(1,2)},S_3^{(1,4)}\}&:\qquad  & \d\Phi_{C_{13}S_3}(b_{13}Q^2,a_{3})\,\d\Phi_{C_{24}S_4}(b_{24}Q^2,a_{34})\nn\\
%   \{C_{134},C_{13},S_{34}^{(1,2)},S_3^{(1,4)}\} &:\qquad  & \d\Phi_{C_{\t{13}4}S_4}(b_{134}Q^2,a_{34})\,\d\Phi_{C_{13}S_3}(b_{13}Q^2,a_3)\nn\\
%   \{C_{134},C_{13},S_{34}^{(1,2)},S_4^{(2,3)}\} &:\qquad  & \d\Phi_{C_{\t{13}4}S_4}(b_{134}Q^2,a_{4}z_3)\,\d\Phi_{C_{13}S_3}(b_{13}Q^2,a_{34})\nn\\  
%   \{C_{134},C_{34},S_{34}^{(1,2)},S_3^{(1,4)}\} &:\qquad  & \d\Phi_{C_{1\t{34}}S_{\t{34}}}(b_{134}Q^2,a_{34})\,\d\Phi_{C_{34}S_3}(b_{34}Q^2,a_{3})\nn\\
%   \eea
% \bea
%   \{C_{12}\}&:\qquad  &\d\Phi_{C_{12}}(b_{12})\nn\\
%   \{C_{134}\}&:\qquad  &\d\Phi_{C_{134}}(b_{134})\nn\\
%   \{S_1^{(2,3)}\}&:\qquad  &\d\Phi_{S_{1}}^{(2,3)}(a_{1},s_{23})\nn\\
%   \{S_{34}^{(1,2)}\}&:\qquad  &\d\Phi_{S_{34}}^{(1,2)}(a_{34},s_{12})\nn\\
%   \{C_{134},S_{34}^{(1,2)}\}&:\qquad  &\d\Phi_{C_{134}S_{34}}(b_{134},a_{34})\nn\\
%   \{C_{12},S_1^{(2,3)}\} &:\qquad  &\d\Phi_{C_{12}S_1}(b_{12},a_1)\nn\\
%   \{S_{34}^{(1,2)},S_{3}^{(1,4)}\}&:\qquad  &\d\Phi_{S_{3}}^{(1,4)}(a_{3},s_{14})\,d\Phi_{S_{4}}^{(1,2)}(a_{34},s_{12})\nn\\
%   \{C_{13}, S_4^{(2,3)}\} &:\qquad  &\d\Phi_{C_{13}}(b_{13})\,\d\Phi_{S_{4}}^{(2,z_3\t{13})}(a_{4},z_3s_{\t{13}2})\nn\\  
%   \{C_{13}, C_{24}\}&:\qquad  &\d\Phi_{C_{13}}(b_{13})\,\d\Phi_{C_{24}}(b_{24})\nn\\
%   \{C_{134},C_{13}\}&:\qquad  &\d\Phi_{C_{\t{13}4}}(b_{134})\,\d\Phi_{C_{13}}(b_{13})\nn\\
%   \{C_{13},S_{34}^{(1,2)}\} &:\qquad  & \d\Phi_{C_{13}S_{3}}(b_{13},a_{34})\,\d\Phi_{S_4}^{(2,\t{13})}(a_{34}-z_3,s_{\t{13}2})\nn\\
%   \{C_{134},S_3^{(1,4)}\}&:\qquad  &\d\Phi_{C_{14}}(b_{134})\,\d\Phi_{S_3}^{(1,4)}(a_3,s_{14})\nn\\
%   \{C_{134},S_4^{(2,3)}\}&:\qquad  &\d\Phi_{C_{13}}(b_{134})\,\d\Phi_{C_{\t{13}4}S_4}(b_{134}-s_{13},z_3 a_4)\nn\\  
%   \{C_{34},S_{34}^{(1,2)}\}&:\qquad  & \d\Phi_{C_{34}}(b_{34})\,\d\Phi_{S_{\t{34}}}^{(1,2)}(a_{34},s_{12})\nn\\
%   \{C_{13}, C_{24},S_3^{(1,4)}\}&:\qquad  & \d\Phi_{C_{13}S_3}(b_{13},a_3)\,\d\Phi_{C_{24}}(b_{24})\nn\\
%   \{C_{13}, C_{24},S_{34}^{(1,2)}\}&:\qquad  & \d\Phi_{C_{13}S_3}(b_{13},a_{34}-z_4)\,\d\Phi_{C_{24}S_4}(b_{24},a_{34})\nn\\
%   \{C_{34},S_{34}^{(1,2)},S_{3}^{(1,4)}\}&:\qquad  & \d\Phi_{C_{34}S_3}(b_{34},a_3)\,\d\Phi_{S_{\t{34}}}^{(1,2)}(a_{34},s_{12})\nn\\
%   \{C_{134},C_{13},S_{3}^{(1,4)}\}&:\qquad  &\d\Phi_{C_{\t{13}4}}(b_{134}) \d\Phi_{C_{13}S_3}(b_{13},a_3)\nn\\
%   \{C_{134},C_{13},S_{4}^{(2,3)}\}&:\qquad  & \d\Phi_{C_{\t{13}4}S_4}(b_{13},z_3a_4)\,\d\Phi_{C_{13}}(b_{134})\nn\\
%   \{C_{134},C_{13},S_{34}^{(1,2)}\}&:\qquad  & \d\Phi_{C_{\t{13}4}S_4}(b_{134},a_{34})\,\d\Phi_{C_{13}S_3}(b_{13},a_{34}-z_4)\nn\\  
%   \{C_{134},C_{34},S_{34}^{(1,2)}\}&:\qquad  & \d\Phi_{C_{1\t{34}}S_{\t{34}}}(b_{134},a_{34})\,\d\Phi_{C_{34}}(b_{34})\nn\\
%   \{C_{134},S_{34}^{(1,2)},S_3^{(1,4)}\}&:\qquad  & \d\Phi_{C_{14}S_4}(b_{134},a_{34})\,\d\Phi_{S_3}^{(1,4)}(a_3,s_{14})\nn\\
%   \{C_{134},S_{34}^{(1,2)},S_4^{(2,3)}\}&:\qquad  & \d\Phi_{C_{13}S_3}(b_{134},a_{34})\,\d\Phi_{C_{14}S_4}(b_{134}-s_{13},z_3a_4)\nn\\
%   \{C_{13},S_{34}^{(1,2)},S_3^{(1,4)}\} &:\qquad  & \d\Phi_{C_{13}S_{3}}(b_{13},a_{3})\,\d\Phi_{S_4}^{(2,\t{13})}(a_{34},s_{\t{13}2})\nn\\
%   \{C_{13},S_{34}^{(1,2)},S_4^{(2,3)}\} &:\qquad  & \d\Phi_{C_{13}S_{3}}(b_{13},a_{34})\,\d\Phi_{S_4}^{(2,z_3\t{13})}(a_{4},z_3s_{\t{13}2})\nn
%     \eea
%   \bea
%   \{C_{13}, C_{24},S_{34}^{(1,2)},S_3^{(1,4)}\}&:\qquad  & \d\Phi_{C_{13}S_3}(b_{13},a_{3})\,\d\Phi_{C_{24}S_4}(b_{24},a_{34})\nn\\
%   \{C_{134},C_{13},S_{34}^{(1,2)},S_3^{(1,4)}\} &:\qquad  & \d\Phi_{C_{\t{13}4}S_4}(b_{134},a_{34})\,\d\Phi_{C_{13}S_3}(b_{13},a_3)\nn\\
%   \{C_{134},C_{13},S_{34}^{(1,2)},S_4^{(2,3)}\} &:\qquad  & \d\Phi_{C_{\t{13}4}S_4}(b_{134},a_{4}z_3)\,\d\Phi_{C_{13}S_3}(b_{13},a_{34})\nn\\  
%   \{C_{134},C_{34},S_{34}^{(1,2)},S_3^{(1,4)}\} &:\qquad  & \d\Phi_{C_{1\t{34}}S_{\t{34}}}(b_{134},a_{34})\,\d\Phi_{C_{34}S_3}(b_{34},a_{3})\nn\\
%   \eea
% The distribution of the (unique) $\Theta$-functions, which categorize a certain limit, over the primitive asymptotic phase space measures is not always unique, and we have made convenient choices when required.














